A Blind Search for Bursts of Very High Enery Gamma Rays with Milagro

Milagro is a water-Cherenkov detector that observes the extended air showers produced by cosmic gamma rays of energies E>100GeV. The effective area of Milagro peaks at energies E~10TeV, however it is still large even down to a few hundred GeV (~10m^2 at 100GeV). The wide field of view (~2sr) and high duty cycle (>90%) of Milagro make it ideal for continuously monitoring the overhead sky for transient Very High Energy (VHE) emissions. This study searched the Milagro data for such emissions. Even though the search was optimized primarily for detecting the emission from Gamma-Ray Bursts (GRBs), it was still sensitive to the emission from the last stages of the evaporation of Primordial Black Holes or to any other kind of phenomena that produce bursts of VHE gamma rays. Measurements of the GRB spectra by satellites up to few tens of GeV showed no signs of a cutoff. Even though multiple instruments sensitive to $GeV/TeV$ gamma rays have performed observations of GRBs, there has not yet been a definitive detection of such an emission yet. One of the reasons for that is that gamma rays with energies E>~100GeV are attenuated by interactions with the extragalactic background light or are absorbed internally at the site of the burst. There are many models that predict VHE gamma-ray emission from GRBs. A detection or a constraint of such an emission can provide useful information on the mechanism and environment of GRBs. This study performed a blind search of the Milagro data of the last five years for bursts of VHE gamma rays with durations ranging from 100musec to 316sec. No GRB localization was provided by an external instrument. Instead, the whole dataset was thoroughly searched in time, space, and duration. No significant events were detected. Upper limits were placed on the VHE emission from GRBs.

==> Chapters/APP_BinSize.tex <==
%Appendix
\appendix
\renewcommand{\thechapter}{A}

\chapter{\label{APP_Binsize}Optimum Bin-Size for Gaussian Statistics}

In this chapter, the optimum bin size will be calculated for the case of large statistics 
of the background and the signal.
This calculation is valid for the searches of durations greater than about $100\,s$. In the case that:

\begin{enumerate}
\item The background distribution is uniform. 
\item The number of signal $(N_{S}$) and background $(N_{BG}$) events
follow a Gaussian distribution: $\left\{ N_{BG},N_{S}\right\} \gg1$. 
\item The statistical fluctuations of the number of background and signal
events are negligible: $\left\{ N_{BG},N_{S}\right\} \gg\left\{ \sqrt{N_{BG}},\sqrt{N_{S}}\right\} $. 
\end{enumerate}
the probability that the number of signal events in a bin were created
by just a background fluctuation can be approximated, similarly to equation \vref{eq:SEARCH_Poisson Probability}, by the cumulative
Gaussian probability: \begin{equation}
P_{G,C}(N_{BG},N_{S})=\int_{N_{S}}^{\infty}\frac{1}{\sqrt{2\pi N_{BG}}}e^{-\frac{\left(N_{S}-N_{BG}\right)^{2}}{2N_{BG}}}\label{eq:GaussianCProb}\end{equation}
The measure of the consistency of a result with the null hypothesis
can be given either by the probability $P_{G,C}$ or by the ``Significance'' $\mathcal{S}$
of the measurement, which is equal to the number of signal events measured
in units of standard deviations of the background:
\begin{equation}
\mathcal{S}\equiv\frac{N_{meas.}-\hat{N}_{BG}}{\sigma(\hat{N}_{BG})}=\frac{(N_{S}+N_{BG})-\hat{N}_{BG}}{\sigma(\hat{N}_{BG})}\simeq\frac{N_{S}+\hat{N}_{BG}-\hat{N}_{BG}}{\sqrt{\hat{N}_{BG}}}=\frac{N_{S}}{\sqrt{\hat{N}_{BG}}}\label{eq:Significance}\end{equation}
As shown in figure \vref{fig:Milagro_delAngle}, the reconstructed directions of the signal events
are distributed according to the point-spread function (PSF) of the detector,
and the reconstructed directions of the background events
are assumed to be distributed locally uniformly. Let us define the efficiency of
including the signal events in a square bin of width $w$, and area
$A=w^{2}$ as $\epsilon(w)$, the background rate per unit area as
$R$, the duration searched as $T$, and the total number of signal
events in the Milagro data as $N_{S,total}$. Then, the number of
signal events and background events included in a bin of width $w$
are $N_{S}(w)=N_{S,total}\,\epsilon(w)$ and $\hat{N}_{BG}(w)=R\,T\,A=R\,T\,w^{2}$
respectively. Equation \ref{eq:Significance} then becomes

\begin{equation}
\mathcal{S}(w,T)=\frac{N_{s}(w)}{\sqrt{\hat{N}_{BG}(w)}}=\frac{N_{S,total}}{\sqrt{R\,T}}\,\frac{\epsilon(w)}{\sqrt{w^{2}}}=\frac{N_{S,total}}{\sqrt{R\,T}}\,\frac{\epsilon(w)}{w}\label{eq:Binsize_significance2}\end{equation}
We see that the significance is a function of the bin width $w$.
In order to maximize the significance, one has to maximize the ratio
$\frac{\epsilon(w)}{w}$. Note that the optimum bin size does not
depend on the background rate $R$ or the total amount of signal $N_{S,total}$.
Because of that, the bin size that maximizes the average significance\footnote{averaged over 
all the possible fluctuations in the conversion from an incoming gamma-ray signal
to Milagro signal events} that corresponds to an incoming gamma-ray signal is equal to
the one that maximizes the detection probability of detecting the same gamma-ray signal.
Therefore, for the case of large statistics, the bin size optimization (maximization of the detection probability) can be 
performed in terms of finding the bin size that maximizes the significance. 

In the following, an analytic bin-size optimization will be presented for the generic case of a 
PSF that follows a Gaussian distribution for both square and round bins (subsecs.
\ref{subsec:CIRC_GAUSS} and \ref{subsec:SQ_GAUSS}), and a numerical bin-size optimization
for a PSF of arbitrary shape and a square bin will be presented in subsection \ref{subsec:BINSIZE_SQGAUSS}. The
results from the last calculation are specific to this study and are to be
used for verification of the Poisson-based 
calculation performed in section \ref{sec:BINSIZE_Poisson}.


\section{\label{subsec:CIRC_GAUSS}Circular Bin and Gaussian PSF}
Consider the case of circular bins and for a PSF that follows
a Gaussian distribution of standard deviation $\sigma$.
The number of expected signal and
background events within a bin of radius $R$ are proportional to:\begin{alignat}{1}
\begin{array}{ccll}
\hat{N}_{S} & \propto & \int_{0}^{R}\frac{e^{-r^{2}/2\sigma^{2}}}{\sigma\sqrt{2\pi}}r & dr\\
\hat{N}_{BG} & \propto & \int_{0}^{R}2\pi & dr\end{array}\label{eq:BINSIZE_CircularBinsOptimization}\end{alignat}
The optical bin size $R_{0}$ maximizes the significance $\hat{N}_{S}/\sqrt{\hat{N}_{BG}}$
so that:
\begin{equation}
\frac{d}{dR}\left\{ \frac{\hat{N}_{S}}{\hat{N}_{BG}}\right\} =0\end{equation}
Using equation \ref{eq:BINSIZE_CircularBinsOptimization} and substituting
$x=r^{2}/\sigma^{2}$ we obtain:
\begin{eqnarray}
\frac{dX}{dR}\frac{d}{dX}\left\{ \frac{\int_{0}^{X}e^{-x/2}dx}{\sqrt{\int_{0}^{X}dx}}\right\}  & = & 0\end{eqnarray}
Since non zero bins $dX/dR\ne0$ therefore:
\begin{eqnarray}
\frac{d}{dX}\left\{ \frac{2\,(1-e^{-X/2})}{\sqrt{X}}\right\}  & = & 0\Rightarrow\\
1+X_{0} & = & e^{X_{0}/2}\Longrightarrow\\
X_{0} & = & 2.513\Longleftrightarrow\\
\mathbf{\mathrm{R_{0}}} & = & 1.585\sigma\label{eq:BINSIZE_OptimumCircular}\end{eqnarray}


\section{\label{subsec:SQ_GAUSS}Square Bin and Gaussian PSF}
For a square bin and a Gaussian PSF, the optimum bin
size can be calculated following a procedure similar to the one above.
In this case:
\begin{alignat}{1}
\begin{array}{ccll}
\hat{N}_{S} & \propto & \int_{-W}^{+W}\int_{-W}^{+W}\frac{e^{-x^{2}/2\sigma^{2}}}{\sigma\sqrt{2\pi}}\,\frac{e^{-y^{2}/2\sigma^{2}}}{\sigma\sqrt{2\pi}} & dxdy\\
\hat{N}_{BG} & \propto & \int_{-W}^{+W}\int_{-W}^{+W}1 & dxdy\end{array}\label{eq:BINSIZE_SquareBinsOptimization}\end{alignat}
If the optimum half width is $W_{0}$ then:
\begin{eqnarray}
0 & = & \frac{d}{dW}\left\{ \frac{\hat{N}_{S}}{\sqrt{\hat{N}_{BG}}}\right\} \\
 & = & \frac{d}{dW}\left\{ \frac{erf\left(\frac{W}{\sqrt{2}\sigma}\right)^{2}}{2W}\right\} \\
 & = & \frac{\sqrt{2}\,erf(\frac{W_{0}}{\sqrt{2}\sigma})e^{-\frac{W_{0}^{2}}{2\sigma^{2}}}}{W_{0}\sqrt{\pi}}-\frac{1}{2}\frac{erf\left(\frac{W_{0}}{\sqrt{2}\sigma}\right)^{2}}{W_{0}^{2}}\end{eqnarray}
This can be solved numerically giving 
\begin{equation}
W_{0}=1.40\,\sigma\simeq\sqrt{2}\,\sigma\label{eq:BINSIZE_OptimumSquare}\end{equation}
It should be noted that equations \ref{eq:BINSIZE_OptimumCircular} and \ref{eq:BINSIZE_OptimumSquare}
say that the area of an optimal circular bin is almost the
same to the area of an optimal square bin (less than $1\%$ difference).


\section{\label{subsec:BINSIZE_SQGAUSS}Square Bin and Non-Gaussian PSF}

In the case that the PSF of the detector does not exactly follow a
Gaussian distribution, the optimum bin size can be calculated numerically
by finding the bin size that maximizes the significance ratio $\hat{N}_{S}/\sqrt{\hat{N}_{BG}}$
of equation \ref{eq:Binsize_significance2}.


In figure \ref{fig:binsize_gaussian}, this ratio is plotted versus
the square bin half-width. Because the angular resolution of the detector
becomes worse with increasing zenith angles, the significance acquires
a dependence on the zenith angle. However, this effect is very
small so the optimum bin half-width is almost the same for all three zenith
angle regions, and equal to $\sim0.8^{o}$. If the PSF of Milagro followed a Gaussian distribution, this optimum bin size
would correspond to a standard deviation of $\sigma=0.8/1.4=0.57^{0}$ (according to eq. 
\ref{eq:BINSIZE_OptimumSquare}).

The angular resolution of the detector
has, a stronger dependence on the properties of the gamma-ray
signal being detected. This analysis used a gamma-ray signal on an
power-law energy spectrum with index -2.2 and with an attenuation
due to interactions with the IR background for a source at a redshift $z=0.2$. 


\begin{figure}[ht]
\includegraphics[width=1\columnwidth]{Plots/Binsize/binsize_gaussian}
\caption{\label{fig:binsize_gaussian}The ratio $\frac{\epsilon(w)}{w}$ found
in the significance formula (eq. \ref{eq:Binsize_significance2})
plotted versus the bin half-width $(w/2)$ for three zenith-angle
regions. The optimum bin half-width corresponds to the peaks of the curves
and is equal to $\sim0.8^{o}$ for all three curves. Data from the Monte Carlo simulation
of the detector were used to construct these plots.}
\end{figure}



==> Chapters/Bibliography.tex <==
\begin{thebibliography}{99}
\setlength{\parskip}{1em}
\end{thebibliography}



==> Chapters/Foreword.tex <==
%Foreword

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{-.65in}

\begin{center}
\large{Foreword} 
\end{center} 

for(e)word plz


==> Chapters/Introduction.tex <==
\chapter{Introduction}
\label{ch:intro}

blabla great thesis
